Visualizing Self-Regulated Learner Profiles in Dashboards: Design Insights from Teachers

Flipped Classrooms (FC) are a promising teaching strategy, where students engage with the learning material before attending face-to-face sessions. While pre-class activities are critical for course success, many students struggle to engage effectively in them due to inadequate of self-regulated learning (SRL) skills. Thus, tools enabling teachers to monitor students' SRL and provide personalized guidance have the potential to improve learning outcomes. However, existing dashboards mostly focus on aggregated information, disregarding recent work leveraging machine learning (ML) approaches that have identified comprehensive, multi-dimensional SRL behaviors. Unfortunately, the complexity of such findings makes them difficult to communicate and act on. In this paper, we follow a teacher-centered approach to study how to make thorough findings accessible to teachers. We design and implement FlippED, a dashboard for monitoring students' SRL behavior. We evaluate the usability and actionability of the tool in semi-structured interviews with ten university teachers. We find that communicating ML-based profiles spark a range of potential interventions for students and course modifications.

==> sections/glossary.tex <==
Co-design is the act of creating with stakeholders (business or customers) specifically within the design development process to ensure the results meet their needs and are usable.

Participatory Design (also often referred to as co-design) looks to actively involve stakeholders, end-users and the wider project team in the design process. 

==> sections/notes.tex <==
%% Lenght of paper
1. Longer intro 

## Methods
1. Change order, SRL profiles first
2. All headings are matching from figure 
3. Check how Tanja cited previous work 


## Structure
1. All the methodology (participants) in the methods

4.1 explain the procedure more

Results for study 1: Log in all the results. How can we group it. Have a table or visualization of results. Table of demographics and results (?).
Visualization of time series.

Results study 2: correlate what they answered and how they explored. topics that they mentioned


Keep the discussion, general guidelines (design guidelines) if you target.
Put everything together. 

Get the best out and then she shorten



==> sections/old/02-method.tex <==
\section{Methodology}
To study how to best communicate online student behavior with teachers, we followed the educator-centered approach shown in Figure \ref{fig:method}. We first conducted ten contextual interviews with university teachers to understand their needs and requirements in the context of FC. Next, we designed graphs according to the users' requirements and previous work on visual designs \cite{gleicher2011visual,albers2014task, lee2016vlat}. To study the preferences of educators, we conducted a visualization study with 100 teachers (See Section \ref{sec:vis-study}). Afterward, we implemented the findings from the visualization study and adapted the graphs accordingly. In parallel, we designed a dashboard and then integrated the graphs resulting from the visualization study. We iteratively tested and modified the dashboard prototype with seven different university teachers. Finally, we evaluated the latest version of the dashboard with ten university teachers in a usability study (See Section \ref{sec:dash-study}). \\

% trim=left bottom right top  \fbox
\begin{figure}
    \centering 
    %\includegraphics[clip, trim=4.7cm 11.7cm 9.7cm 6.0cm, width=1\textwidth]{figures/method-3.pdf}
    \includegraphics[width=0.8\textwidth]{figures/method-8.png}
    \caption{Educator-centered approach}
    \label{fig:method}
\end{figure}

\noindent \textbf{ML-Assisted Analysis}
We recorded with consent all the semi-structured interviews (contextual interviews and user studies) and transcribed them using \texttt{Whisper} \cite{radford2022robust}, a state-of-the-art zero-shot model for speech recognition. We then performed the qualitative analysis assisted by topic modeling. We identified the main topics using \texttt{BERTopic}~\cite{grootendorst2022bertopic}, a topic modeling technique that integrates the contextual information of the text by clustering embeddings generated by pre-trained Transformer-based language models. In particular, we generated the embeddings using \texttt{Sentence-BERT}~\cite{reimers2019sentence}. The code and supplementary materials (e.g., interview protocols) are available at \url{https://anonymous.4open.science/r/flipped/}. \\


\subsection{Contextual Understanding} 
\label{sec:context}

%% Introduce clustering pipeline (?)
\noindent \textbf{SRL Profiles}. 
Recent work on BL and student behavior has focused on students' studying habits and SRL patterns \cite{saint2020, mejia-domenzain_identifying_2022}. \cite{mejia-domenzain_identifying_2022} studied SRL through 5 different lenses: \textit{Effort}, \textit{Consistency}, \textit{Regularity}, \textit{Control}, and \textit{Proactivity}. Different patterns of behaviors were identified using a multi-step time series clustering pipeline that takes as input clickstream features from a learning management system (LMS). The five lenses were integrated into multi-dimensional student profiles that are correlated with academic performance. Technically, \cite{mejia-domenzain_identifying_2022} measured \textit{Effort} with the time online and clicks on videos; \textit{Consistency} with the mean session duration and relative time online; \textit{Regularity} with the day-of-the-week and hour-of-the-day periodicity; \textit{Proactivity} with the delay or anticipation to watch the lecture content; and \textit{Control} using the pause frequency and the changes in video speed. In the pipeline, they (1) calculate the dynamic time-warping distance between the students' time series features, (2) add the distances from the features in the same dimension, and (3) use Spectral Clustering to find the different groups per dimension. In a second clustering step, the resulting labels per dimension (5 labels) are clustered using K-Modes. In our work, we adapt the clustering pipeline from \cite{mejia-domenzain_identifying_2022} to study how to communicate and visualize students' behaviors and ML-based profiles. \\


\noindent \textbf{User Interviews}. We conducted semi-structured interviews with ten teachers at university level (50\% of the teachers identified as female). The median time of the interviews was 40 minutes. Participants were asked about their experience with blended learning and the challenges they encountered. Then, they were asked about the information they would have liked to know and how would they have liked to see or receive that information. Lastly, they were asked to make a sketch and draw how they would like the information to be visualized and organized.\\

\noindent \textbf{Findings}. 90\% of the teachers interviewed agreed that having data about their students' learning behaviors would help them adapt their course and give personalized feedback to specific student profiles. The most mentioned requirement (by 80\% of educators) was anonymous data and aggregated statistics. Educators were concerned about data privacy and shared ethical concerns. However, they showed interest in general group statistics. For example, 60\% of the interviewees mentioned it would be useful to know whether students viewed the material, how much time they spent watching the videos, and the number of students keeping up with the class. Some other mentions were students’ consistency in watching the videos, whether students worked at the last minute before an exam, and the average video playback speed. \\ 




\begin{comment}
    
\subsection{Visual Design Teacher Preferences} 
\label{sec:vis-method}

%% Participants
\noindent \textbf{Participants}.We recruited $100$ participants using Prolific, prescreening participants fluent in English and that taught in the education industry. We removed 8 participants that failed the attention checks. In addition, we requested a balanced sample of male and female participants (51\% female). The age of the respondents ranged between 21 and 76 years old, with a median of 37 years old. 68\% of the participants came from Europe and more precisely 41\% from the United Kingdom. 34\% of the participants reported teaching at university, 29\% at high school, 23\% at elementary school, and the remaining 14\% included kindergarten, adult education, and vocational education. We found that only 35\% of the university teachers were female. \\


%% Explain the survey (procedure)
\noindent \textbf{Procedure}. Participants were given the scenario of teaching a large university course for bachelor students in a flipped manner. They were told they had taught 2/3 of the course and would be shown visualizations of their students' SRL behavior. Next, the participants were shown, in random order, graphs corresponding to each of the SRL dimensions \cite{mejia-domenzain_identifying_2022}. Per visualization, participants were asked to (1) describe and analyze the graph as if they had to explain it to a visually impaired colleague (the descriptions were used to generate the captions and alt-text), (2) explain their insights, and (3) suggest how to improve the graph (optional). In addition, to measure visualization literacy\cite{lee2016vlat}, we asked participants to solve four tasks adapted from VLAT \cite{lee2016vlat}: retrieve values (item 55), find extremum (item 2), find trend (item 38), and make comparisons with relative values (item 15).

\begin{figure}
    \centering
%\includegraphics[width=1.00\textwidth]{figures/plots_examples.png}
    \includegraphics[clip, trim=0.3cm 0.35cm 0.25cm 0.25cm, width=1\textwidth]{figures/plots_examples.pdf}
    \caption{Examples of time series visual designs explored in the survey.}
    \label{fig:rank-effort}
\end{figure}

Furthermore, we asked participants to rank in ascending order (rank 1 is the highest and best) different types of graphs for a single feature according to their usefulness and explain the rationale for their preference. Similar to \cite{albers2014task}, we visualized time series using different designs and graph types. For example, Figure \ref{fig:rank-effort} shows a bar plot, line plot, box plot, and heat map to represent the time the students spent on online activities through time. We explored other visual designs for the evolution of groups (e.g., stacked area graph, bubble graph, and Sankey flow graph in Figure \ref{fig:rank-profiles}) and design decisions including whether it is more useful to show the relative or the absolute number of students, and use of legends\footnote{The complete protocol is available in the supplementary materials.}. Lastly, like \cite{gleicher2011visual}, we explored comparative designs of multiple time series including juxtaposition, superposition, and explicit encoding of relationships.
% trim=left bottom right top  \fbox
\begin{figure}
    \centering
    \includegraphics[clip, trim=0.9cm 18.3cm 2.8cm 2.0cm, width=1\textwidth]{figures/profiles-examples.pdf}
    \caption{Examples of charts for the evolution of groups explored in the survey.}
    \label{fig:rank-profiles}
\end{figure}


%Visual Design Teacher Preferences
\subsection{Teacher Dashboard for SRL Profiles} 
\label{sec:dash-method}

% trim=left bottom right top  \fbox
\begin{figure}
    \centering
    %\includegraphics[clip, trim=0.1cm 5.1cm 0cm 5.1cm, width=1\textwidth]{figures/overview.pdf}
    \includegraphics[width=1\textwidth]{figures/dashboard-design.png}
    \caption{Overview of pages: (a)\textit{Summary}, (b)\textit{Student Profiles}, (c) \textit{Effort} and (d) \textit{Effort groups} .}
    \label{fig:overview}
\end{figure}


\noindent \textbf{Design}. From the potential user interviews, we designed and implemented a prototype of \texttt{FlippED}. The design includes a navigation menu (see F1 in Figure \ref{fig:overview}) with two parts: the overview (with the \textit{Summary} and the \textit{Student Profiles}) and the student behaviors (including \textit{Proactivity, Effort, Consistency, Control} and \textit{Regularity}). The user can select the course (F2) and the date range (F3). In addition, there are help buttons (F4) throughout the dashboard to clarify the different elements and to provide further explanations. Figure \ref{fig:overview} shows the two overview pages. In the \textit{Summary} page (left on Figure \ref{fig:overview}), weekly statistics per dimension are displayed as well as the trend in comparison to the previous week. The description of the profiles and the associated grades are shown on the \textit{Profiles} page (Figure \ref{fig:overview}b). Moreover, Figure \ref{fig:overview}c and \ref{fig:overview}d  show examples of the student behavior pages in which users can choose (F5) between the aggregated view (\ref{fig:overview}c) and a view per groups (\ref{fig:overview}d).




The online interaction flow (see Figure \ref{fig:interaction-flow}) consists of retrieving the graphs, text, and captions from the database. Offline, the content retrieval backend obtains the students' clickstream data from the LMS and runs the clustering pipeline. The results are used to generate the graphs, text, and captions which are then stored in the database to be retrieved in real-time. \\

% trim=left botm right top  \fbox
\begin{figure}
    \centering
    \includegraphics[clip, trim=1.9cm 12cm 5.5cm 6.3cm, width=1\textwidth]{figures/interaction.pdf}
    \caption{Interaction flow.}
    \label{fig:interaction-flow}
\end{figure}

\noindent \textbf{Accessibility.} In order to make \texttt{FlippED} accessible to people with disabilities, we followed the guidelines from the \textit{Web Accessibility Initiative (WAI)} \cite{wai} and achieved the conformance level of AAA\footnote{The evaluation report is available in the supplementary materials.} (highest level). Some examples of accessible features include: using a colorblind palette and providing detailed alt-texts, and captions for all graphs; supporting dark contrast mode; and having a clear voice-navigable interface. 
The interface (front-end) was implemented with React and the content retrieval (back-end) with FastAPI using a Postgres database. Both applications were hosted on Heroku.


\noindent \textbf{Participants}. We recruited 10 university-level teachers with experience in BL (6 had experience teaching FC), through a faculty email and LinkedIn posts. 50\% of the teachers were female. \\

%% Explain the survey (procedure)
\noindent \textbf{Procedure}. At the beginning of the user study, participants filled out a questionnaire about their trust in AI-based educational technology (EdTech). We used constructs 1, 3, and 5 (self-efficacy, anxieties, and benefits regarding AI-based EdTech) from \cite{nazaretsky_instrument_2022}. We then conducted semi-structured interviews where participants were given the same scenario from the visualization study: teaching a large FC university course. The first task was to follow a think-aloud protocol and explore the dashboard. After the exploration, participants were told that students had just taken their midterm exam and the results were surprisingly bad for some students. The second task was to use the dashboard to give possible explanations. Lastly, we asked participants to assess whether they would use it and how they would use it.

\subsection{Measures and Analysis}


\noindent \textbf{ML-Assisted Analysis}
We recorded with consent all the semi-structured interviews (contextual interviews and user studies) and transcribed them using \texttt{Whisper} \cite{radford2022robust}, a state-of-the-art zero-shot model for speech recognition. We then performed the qualitative analysis assisted by topic modeling. We identified the main topics using \texttt{BERTopic}~\cite{grootendorst2022bertopic}, a topic modeling technique that integrates the contextual information of the text by clustering embeddings generated by pre-trained Transformer-based language models. In particular, we generated the embeddings using \texttt{Sentence-BERT}~\cite{reimers2019sentence}. The code and supplementary materials (e.g., interview protocols) are available at \url{https://anonymous.4open.science/r/flipped/}. \\

\noindent \textbf{Ranking Analysis.} For the Visual Design Teacher Preferences, we analyzed the preferences differences based on demographic (sex and age) and personal factors (teaching level). We used the non-parametric test \textit{Kruskal–Wallis} to evaluate the ordinal rankings. When significant, we performed a pairwise comparison using the \textit{Mann-Whitney U} test, correcting for multiple comparisons via a \textit{Benjamini-Hochberg (BH)} procedure.
\end{comment}
 


==> sections/old/03-results.tex <==
%% Results
\section{Results}

We evaluated ou

%% Research question 1: Visualization Study 
\subsection{Visualization Study}

%% Table reporting demographics

%% Best Visualizations 

%% Research question 2: Dashboard Study 
\subsection{Dashboard Study}

% trim=left botm right top  \fbox
\begin{figure}
    \centering
    \includegraphics[clip, trim=0.2cm 4.9cm 0.3cm 5.0cm, width=1.00\textwidth]{figures/effort.pdf}
    \caption{Performance on recipe task and transfer task. Error bars showing the standard deviation.}
    \label{fig:performance}
\end{figure}

% trim=left botm right top 
\begin{figure}
    \centering
    \includegraphics[clip, trim=1cm 0cm 1cm 1cm, width=1\textwidth]{figures/flow.pdf}
    \caption{Performance on recipe task and transfer task. Error bars showing the standard deviation.}
    \label{fig:performance}
\end{figure}

==> sections/old/03-vis-complete.tex <==
%% Explain the survey (procedure)
\noindent \textbf{Procedure}. Participants were given the scenario of teaching a large university course for bachelor students in a flipped manner. They were told they had taught 2/3 of the course and would be shown visualizations of their students' SRL behavior. Next, the participants were shown, in random order, graphs corresponding to each of the SRL dimensions \cite{mejia-domenzain_identifying_2022}. Per visualization, participants were asked to (1) describe and analyze the graph as if they had to explain it to a visually impaired colleague (the descriptions were used to generate the captions and alt-text), (2) explain their insights, and (3) suggest how to improve the graph (optional). 

%In addition, to measure visualization literacy\cite{lee2016vlat}, we asked participants to solve four tasks adapted from VLAT \cite{lee2016vlat}: retrieve values (item 55), find extremum (item 2), find trend (item 38), and make comparisons with relative values (item 15).


\begin{figure}
    \centering
    %\includegraphics[width=1.00\textwidth]{figures/plots_examples.png}
    \includegraphics[clip, trim=0.3cm 0.35cm 0.25cm 0.25cm, width=1\textwidth]{figures/plots_examples.pdf}
    \caption{Examples of time series charts explored in the survey.}
    \label{fig:rank-effort}
\end{figure}

\input{tables/procedure-vis.tex}


Furthermore, we asked participants to rank in ascending order (rank 1 is the highest and best) different types of graphs for a single feature according to their usefulness and explain the rationale for their preference. Table \ref{tab:procedure} details the evaluation tasks per concept explored\footnote{The complete protocol is available in the supplementary materials.}. 


%Similar to \cite{albers2014task}, we visualized time series using different designs and graph types. For example, Figure \ref{fig:rank-effort} shows a bar plot, line plot, box plot, and heat map to represent the time the students spent on online activities through time. We explored other visual designs for the evolution of groups (e.g., stacked area graph, bubble graph, and Sankey flow graph in Figure \ref{fig:rank-profiles}) and design decisions including whether it is more useful to show the relative or the absolute number of students, and use of legends. Lastly, like \cite{gleicher2011visual}, we explored comparative designs of multiple time series including juxtaposition, superposition, and explicit encoding of relationships\footnote{The complete protocol is available in the supplementary materials.}.


% trim=left bottom right top  \fbox
\begin{figure}
    \centering 
    %\includegraphics[clip, trim=4.7cm 11.7cm 9.7cm 6.0cm, width=1\textwidth]{figures/method-3.pdf}
    \includegraphics[clip,width=1\textwidth]{figures/groups_comp.pdf}
    \caption{Examples of group comparison charts explored in the survey}
    \label{fig:comp}
\end{figure}


% trim=left bottom right top  \fbox
\begin{figure}
    \centering
    \includegraphics[clip, trim=0.9cm 18.3cm 2.8cm 2.0cm, width=1\textwidth]{figures/profiles-examples.pdf}
    \caption{Examples of evolution of groups charts explored in the survey.}
    \label{fig:rank-profiles}
\end{figure}

We analyzed the preferences differences based on demographic (sex and age) and personal factors (teaching level). We used the non-parametric test Kruskal–Wallis to evaluate the ordinal rankings. When significant, we performed a pairwise comparison using the Mann-Whitney U test, correcting for multiple comparisons via a Benjamini-Hochberg procedure.


\subsection{Results}

%% Graph literacy
\noindent \textbf{Graph Literacy}. Participants completed the study in 58 minutes (median time). We computed the visualization literacy score (VL) as a weighted average using as weights the items' discrimination index times the content validity ratio from \cite{lee2016vlat} (0.6 for retrieving the value, 6 for finding extremum, 14 for finding trend, and 6.4 for making comparisons with relative values). The mean VL was 0.7/1.0 ($\sigma$ = 0.3) indicating good literacy. The personal (teaching level) and demographic (gender, age) factors did not explain the variance.  \\


% trim=left bottom right top  \fbox
\begin{figure}
    \centering 
    %\includegraphics[clip, trim=4.7cm 11.7cm 9.7cm 6.0cm, width=1\textwidth]{figures/method-3.pdf}
    \includegraphics[width=1\textwidth]{figures/ranking-results.png}
    \caption{Mean ranking for (a) Time series, and (b) group comparison}
    \label{fig:mean-ranking}
\end{figure}


%% Time series 
\noindent \textbf{Plot Type}. \\
\noindent \textit{Time series}. We found that participants differed in their preferences to visualize time series behavior of students (${\chi}^2(5) = 188$, $p < 0.001$). For example, we used the \textit{Effort} feature of time spent online (e.g., see Figure \ref{fig:rank-effort}) and found that participants preferred (in ascending order where lower is better) bar plot ($\mu_{rank}$= 2.1), followed by bar plot with a line plot on top ($\mu_{rank}$=  2.7), a line plot with standard deviation ($\mu_{rank}$=  3.1), just a line plot ($\mu_{rank}$=  3.3), heat map ($\mu_{rank}$=  4.7) and box plot ($\mu_{rank}$= 4.9). As shown in figure \ref{fig:mean-ranking}a, university teachers ranked the line plot with standard deviation higher ($\mu_{rank}$=  2.7) than the rest of the teachers (${\chi}^2(2) = 4.3$, $p = 0.03$). After the bar plot, it was the preferred plot. One of the main topics when explaining the preferences was \textit{clarity}. This is coherent with the findings from \cite{albers2014task} where the graph that included the bar plot with a line plot on top outperformed the other graphs (line plot, box plot, and heat map) at identifying statistical properties (e.g., range, average, extremes). However, when we analyzed the topics in the written insights derived from the plots, we found two topics (out of 13) unique to the heat map. Participants realized that \textit{usually most students were putting in 0 [effort]} and that \textit{a little amount of them spent a lot of time on the platform}. Although this information could have also been inferred from the line plot with standard deviation and the box plot, it is interesting that it was only mentioned for the heat map. \\

\noindent \textbf{Frequency}. The preferences were similar when visualizing the frequency of events, for example, studying habits according to the day of the week and the time of the day. We found that 84\% of the participants preferred to visualize the frequency of events with a bar plot where the y-axis represented the frequency than with heat maps where the colors and the transparency illustrated the frequency. \\

%% Comparison
\noindent \textbf{Group comparison}. When comparing groups in graphs participants preferred superposition (overlaying objects in the same space) over juxtaposition (showing different objects separately). For example,  with line plots, 84\% of participants preferred superposition over juxtaposition (${\chi}^2(1) = 83$, $p < 0.001$). Likewise, when using bar plots to compare time series (see Figure \ref{fig:comp}), participants also preferred superposition over juxtaposition and the explicit encoding of relationships (${\chi}^2(3) = 67$, $p < 0.001$).  We explored superposition by overlapping objects side-by-side and on top of each other. As seen in Figure \ref{fig:mean-ranking}, side-by-side superposition was preferred ($\mu_{rank}$=  1.9) over juxtaposition ($\mu_{rank}$=  2.4), superposition on top of each other ($\mu_{rank}$=  2.6) and the difference between the time series ($\mu_{rank}$=  3.3). The participants of \textit{younger age} (younger than the 25th percentile of 30 years old) ranked the difference-between-time-series graph higher ($\mu_{rank}$=  2.9) than the rest of the participants ($\mu_{rank}$=  3.3) but it also remained as the lowest ranked. One \textit{young} participant noted that \textit{the difference makes it very simple as it reduces complexity (in terms of elements in the plot)}; this observation is in line with \cite{gleicher2011visual} that argues that explicit encodings can offload the burden of comparison from the viewer. \\

%% composition and comparison of a few variables over time (proactivity)
\noindent \textbf{Composition over time}. We studied the composition over time using stacked bar charts. We used, as example, the proportion of students per week that watched the pre-class videos before and after the interactive session. We found that 87\% of participants preferred having a third group with the students that did not watch the videos so that the bars would add up to the maximum number of students. Despite some participants argued that \textit{it isn't necessary to cluter the graph with that information}, the majority agreed that they \textit{would still prefer to see how many students did not watch than calculate it and add [their] head}. \\

%% Numerical proportion
\noindent \textbf{Numerical proportion}. To show the relative sizes of data, for example, the number of students per cluster at a given point, the pie chart ($\mu_{rank}$=  1.2) was strongly favored over a network graph ($\mu_{rank}$=  2.5), a stacked area graph ($\mu_{rank}$=  2.5), and a bubble chart ($\mu_{rank}$=  3.1). Participants argued that the pie chart \textit{is the most familiar and traditional}.\\


%% Evolution of groups
\noindent \textbf{Evolution of groups}. We compared graphs for the evolution of a numeric variable for several groups (see Figure \ref{fig:rank-profiles}) using a stacked area chart ($\mu_{rank}$=  1.5), a bubble chart ($\mu_{rank}$=  1.9) and a Sankey flow chart ($\mu_{rank}$=  2.6). Noteworthy, the participants of \textit{older age} (older than the 75th percentile of 46 years old) ranked the stacked area chart and the bubble chart equally ($\mu_{rank}$=  1.6), one of them noted \textit{the bubble charts were easier to read and understand the focus}.\\

%% Absolute or relative numbers
\noindent \textbf{Values representation}. Participants were divided between showing the number of students as a percentage (51\%) or in absolute terms (49\%). However, 71\% of university teachers preferred percentages over absolute numbers, and some of them suggested \textit{adding the total number of students to the y-axis label so that it can be calculated with the percentages if desired}. Lastly, when comparing time series, we found that 75\% of the participants favored using legends in graphs.




==> sections/old/03-visualization-simple.tex <==
\section{Study 1: Visual Design Teacher Preferences}
\label{sec:vis-study}

To answer \textbf{RQ1}, we conducted a large-scale study to evaluate teacher visual design preferences for \textit{plot type} of time series, frequency, and categorical features; \textit{group comparison} for time series and frequency data; \textit{plot composition} and \textit{group evolution} of categorical time series; and \textit{value representation} of categorical features.

\subsection{Experimental Setup}

%% Participants
\noindent \textbf{Participants}.We recruited $100$ participants using Prolific, prescreening participants fluent in English and that taught in the education industry. We removed 8 participants that failed the attention checks. In addition, we requested a balanced sample of participants identified as male and female (51\% female). The age of the respondents ranged between 21 and 76 years old, with a median of 37 years old. 68\% of the participants came from Europe and more precisely 41\% from the United Kingdom. 34\% of the participants reported teaching at university, 29\% at high school, 23\% at elementary school, and the remaining 14\% included kindergarten, adult education, and vocational education. We found that only 35\% of the university teachers were female. \\


\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\input{tables/procedure-vis-3.tex}
}
\caption{Concepts explored per feature type with description and tasks.}
\label{tab:procedure}
\end{table}

%% Explain the survey (procedure)
\noindent \textbf{Procedure}. Participants were given the scenario of teaching a large university course for bachelor students in a flipped manner. They were told they had taught 2/3 of the course and would be shown visualizations of their students' SRL behavior. Then, we evaluated the plot type, group comparison, plot composition, group evolution, and value representation with different types of features (see Table \ref{tab:procedure}).


\begin{figure}
    \centering
    %\includegraphics[width=1.00\textwidth]{figures/plots_examples.png}
    \includegraphics[clip, trim=0.3cm 0.35cm 0.25cm 0.25cm, width=1\textwidth]{figures/plots_examples.pdf}
    \caption{Diverse representations of time series.}
    \label{fig:rank-effort}
\end{figure}

First, participants were shown, in random order, different designs of time series (see Figure \ref{fig:rank-effort}), frequency, categorical, and categorical time series (see Figure \ref{fig:rank-profiles})graphs to evaluate the different representations. Per visualization, participants were asked to (1) describe and analyze the graph, (2) explain their insights, and (3) suggest how to improve the graph (optional).  Furthermore, we asked participants to rank in ascending order (rank 1 is the highest and best) the different designs according to their usefulness and explain the rationale for their preference. Similar to \cite{albers2014task}, we visualized time series using different designs and graph types. For example, Figure \ref{fig:rank-effort} shows a bar plot, line plot, box plot, and heat map to represent the time the students spent on online activities through time. 


% trim=left bottom right top  \fbox
\begin{figure}
    \centering
    \includegraphics[clip, trim=0.9cm 18.3cm 2.8cm 2.0cm, width=1\textwidth]{figures/profiles-examples.pdf}
    \caption{Diverse representations of categorical time series explored in the survey.}
    \label{fig:rank-profiles}
\end{figure}


Second, we explored the group comparison with time series and frequency plots. Following group comparison taxonomy\cite{gleicher2011visual}, we explored different comparative layouts including juxtaposition, superposition, and explicit encoding of relationships (e.g., Figure \ref{fig:comp}) \footnote{The complete protocol is available in the supplementary materials.}.

% trim=left bottom right top  \fbox
\begin{figure}
    \centering 
    %\includegraphics[clip, trim=4.7cm 11.7cm 9.7cm 6.0cm, width=1\textwidth]{figures/method-3.pdf}
    \includegraphics[clip,width=1\textwidth]{figures/groups_comp-2.pdf}
    \caption{Examples of group comparison time series charts explored in the survey}
    \label{fig:comp}
\end{figure}
In addition, to measure visualization literacy\cite{lee2016vlat}, we asked participants to solve four tasks adapted from VLAT \cite{lee2016vlat}: retrieve values (item 55), find extremum (item 2), find trend (item 38), and make comparisons with relative values (item 15). We analyzed the preferences differences based on demographic (sex and age) and personal factors (teaching level). We used the non-parametric test Kruskal–Wallis to evaluate the ordinal rankings. When significant, we performed a pairwise comparison using the Mann-Whitney U test, correcting for multiple comparisons via a Benjamini-Hochberg procedure.


\subsection{Results}

%Participants completed the study in 58 minutes (median time).
%% Graph literacy
\noindent \textbf{Graph Literacy}.  We computed the visualization literacy score (VL) as a weighted average using as weights the items' discrimination index times the content validity ratio from \cite{lee2016vlat} (0.6 for retrieving the value, 6 for finding extremum, 14 for finding trend, and 6.4 for making comparisons with relative values). The mean VL was 0.7/1.0 ($\sigma$ = 0.3) indicating good literacy. The personal (teaching level) and demographic (gender, age) factors did not explain the variance.  \\


% trim=left bottom right top  \fbox
\begin{figure}
    \centering 
    %\includegraphics[clip, trim=4.7cm 11.7cm 9.7cm 6.0cm, width=1\textwidth]{figures/method-3.pdf}
    \includegraphics[width=1\textwidth]{figures/results-2.png}
    \caption{Mean ranking for time series representation (a), and group comparison (b). (*) indicates a significant difference with \textit{p}-value $< 0.05$. }
    \label{fig:mean-ranking}
\end{figure}


%% Time series 
\noindent \textbf{\textit{3.2.1 Representation}} \\
\noindent \textbf{Time series}. We found that participants differed in their preferences to visualize time series behavior of students (${\chi}^2(5) = 188$, $p < 0.001$). For example, we used the \textit{Effort} feature of time spent online (e.g., see Figure \ref{fig:rank-effort}) and found that participants preferred (in ascending order where lower is better) bar plot ($\mu_{rank}$= 2.1), followed by bar plot with a line plot on top ($\mu_{rank}$=  2.7), a line plot with standard deviation (SD) ($\mu_{rank}$=  3.1), just a line plot ($\mu_{rank}$=  3.3), heat map ($\mu_{rank}$=  4.7) and box plot ($\mu_{rank}$= 4.9). As shown in figure \ref{fig:mean-ranking}a, university teachers ranked the line plot with SD higher ($\mu_{rank}$=  2.7) than the rest of the teachers (${\chi}^2(2) = 4.3$, $p = 0.03$). After the bar plot, it was the preferred plot. One of the main topics when explaining the preferences was \textit{clarity}. This is coherent with the findings from \cite{albers2014task} where the graph that included the bar plot with a line plot on top outperformed the other graphs (line plot, box plot, and heat map) at identifying statistical properties (e.g., range, average, extremes). However, when we analyzed the topics in the written insights derived from the plots, we found two topics (out of 13) unique to the heat map. Participants realized that \textit{usually most students were putting in 0 [effort]} and that \textit{a little amount of them spent a lot of time on the platform}. Although this information could have also been inferred from the line plot with standard deviation and the box plot, it is interesting that it was only mentioned for the heat map. \\

\noindent \textbf{Frequency}. The preferences were similar when visualizing the frequency of events, for example, studying habits according to the day of the week and the time of the day. We found that 84\% of the participants preferred to visualize the frequency of events with a bar plot where the y-axis represented the frequency than with heat maps where the colors and the transparency illustrated the frequency. \\


%% Numerical proportion
\noindent \textbf{Categorical}. To show the relative sizes of data, for example, the number of students per cluster at a given point, the pie chart ($\mu_{rank}$=  1.2) was strongly favored over a network graph ($\mu_{rank}$=  2.5), a stacked area graph ($\mu_{rank}$=  2.5), and a bubble chart ($\mu_{rank}$=  3.1). Participants argued that the pie chart \textit{is the most familiar and traditional}.\\


%% Evolution of groups
\noindent \textbf{Categorical time series}. We compared graphs for the evolution of a numeric variable for several groups (see Figure \ref{fig:rank-profiles}) using a stacked area chart ($\mu_{rank}$=  1.5), a bubble chart ($\mu_{rank}$=  1.9) and a Sankey flow chart ($\mu_{rank}$=  2.6). Noteworthy, the participants of \textit{older age} (older than the 75th percentile of 46 years old) ranked the stacked area chart and the bubble chart equally ($\mu_{rank}$=  1.6), one of them noted \textit{the bubble charts were easier to read and understand the focus}. Moreover, we also studied the composition over time using stacked bar charts. We used, as example, the proportion of students per week that watched the pre-class videos before and after the interactive session. We found that 87\% of participants preferred having a third group with the students that did not watch the videos so that the bars would add up to the maximum number of students. Despite some participants argued that \textit{it isn't necessary to cluter the graph with that information}, the majority agreed that they \textit{would still prefer to see how many students did not watch than calculate it and add [their] head}. \\

%% Absolute or relative numbers
\noindent \textbf{Values}. Participants were divided between showing the number of students as a percentage (51\%) or in absolute terms (49\%). However, 71\% of university teachers preferred percentages over absolute numbers, and some of them suggested \textit{adding the total number of students to the y-axis label so that it can be calculated with the percentages if desired}. Lastly, when comparing time series, we found that 75\% of the participants favored using legends in graphs.


%% Comparison
\subsubsection{\textit{3.2.2 Group Comparison}}. \\
When comparing groups in graphs participants preferred superposition (overlaying objects in the same space) over juxtaposition (showing different objects separately). For example,  with time series line plots, 84\% of participants preferred superposition over juxtaposition (${\chi}^2(1) = 83$, $p < 0.001$). Likewise, when using bar plots to compare time series (see Figure \ref{fig:comp}), participants also preferred superposition over juxtaposition and the explicit encoding of relationships (${\chi}^2(3) = 67$, $p < 0.001$).  We explored superposition by overlapping objects side-by-side and on top of each other. As seen in Figure \ref{fig:mean-ranking}, side-by-side superposition was preferred ($\mu_{rank}$=  1.9) over juxtaposition ($\mu_{rank}$=  2.4), superposition on top of each other ($\mu_{rank}$=  2.6) and the difference between the time series ($\mu_{rank}$=  3.3). The participants of \textit{younger age} (younger than the 25th percentile of 30 years old) ranked the difference-between-time-series graph higher ($\mu_{rank}$=  2.9) than the rest of the participants ($\mu_{rank}$=  3.3) but it also remained as the lowest ranked. One \textit{young} participant noted that \textit{the difference makes it very simple as it reduces complexity (in terms of elements in the plot)}. However, despite explicit encodings can offload the burden of comparison from the viewer \cite{gleicher2011visual}, the preferred layout for time series was superposition. These findings were also valid for frequency plots where 83\% preferred superposition over juxtaposition.\\


\textit{In summary, teachers tend to prefer simpler and more familiar visualizations like bar plots and pie charts. In addition, when comparing groups the superposition layout was perceived as more useful. We found no differences regarding gender but found that age and teaching level (i.e., university) were correlated with some visual design preferences \textbf{RQ1}.}
 

==> sections/old/03-visualization-study.tex <==
\section{Study 1: Visual Design Preferences of Teachers}
\label{sec:vis-study}

To answer \textbf{RQ1}, we conducted a large-scale study to evaluate teacher visual design preferences for \textit{plot type} of time series, frequency, and categorical features; \textit{group comparison} for time series and frequency data; \textit{group evolution} 
 and \textit{plot composition} of categorical time series; and \textit{value representation} of categorical features.

\subsection{Experimental Setup}

%% Participants
\noindent \textbf{Participants}.We recruited $100$ participants using Prolific, prescreening participants fluent in English and that taught in the education industry. We removed 8 participants that failed the attention checks. In addition, we requested a balanced sample of participants identified as male and female (51\% female). The age of the respondents ranged between 21 and 76 years old, with a median of 37 years old. 68\% of the participants came from Europe and more precisely 41\% from the United Kingdom. 34\% of the participants reported teaching at university, 29\% at high school, 23\% at elementary school, and the remaining 14\% included kindergarten, adult education, and vocational education. We found that only 35\% of the university teachers were female. \\


\begin{table}[]
\centering
%\resizebox{\textwidth}{!}{%
\input{tables/procedure_vis_long.tex}
%}
\caption{Concepts explored per feature type with description and tasks.}
\label{tab:procedure}
\end{table}

%% Explain the survey (procedure)
\noindent \textbf{Procedure}. Participants were given the scenario of teaching a large university course for bachelor students in a flipped manner. They were told they had taught 2/3 of the course and would be shown visualizations of their students' SRL behavior. Then, we evaluated the plot type, group comparison, plot composition, group evolution, and value representation with different types of features (see Table \ref{tab:procedure}).


\begin{figure}
    \centering
    %\includegraphics[width=1.00\textwidth]{figures/plots_examples.png}
    \includegraphics[clip, trim=0.3cm 0.35cm 0.25cm 0.25cm, width=1\textwidth]{figures/plots_examples.pdf}
    \caption{Diverse representations of time series.}
    \label{fig:rank-effort}
\end{figure}

\noindent Participants were shown, in random order, the concepts shown in table \ref{tab:procedure}. They were asked to interpret graphs by (1) describing and analyzing the it, (2) explaining their insights, and (3) suggesting how to improve the it (optional). In addition, we asked participants to rank in ascending order (rank 1 is the highest and best) the different designs according to their usefulness and explain the rationale for their preference. 

\noindent We explored \textit{Plot Type} by evaluating different designs per feature type. For time series and frequency, we adapted the most informative designs from \cite{albers2014task, evergreen_design_2013}. For example, Figure \ref{fig:rank-effort} shows a bar plot, line plot, box plot, and heat map to represent the time the students spent on online activities through time. Moreover, for categorical features, we adapted the chart types from other visualization studies \cite{lee2016vlat}. 


% trim=left bottom right top  \fbox
\begin{figure}
    \centering
    \includegraphics[clip, trim=0.9cm 18.3cm 2.8cm 2.0cm, width=1\textwidth]{figures/profiles-examples.pdf}
    \caption{Diverse representations of categorical time series explored in the survey.}
    \label{fig:rank-profiles}
\end{figure}


\noindent Next, we explored the \textit{group comparison} with time series and frequency plots. Following the group comparison taxonomy \cite{gleicher2011visual}, we explored different comparative layouts including juxtaposition, superposition, and explicit encoding of relationships (e.g., Figure \ref{fig:comp}).  Moreover, we explored other concepts and design decisions like how to visualize group evolution (designs from \cite{lee2016vlat, evergreen_design_2013, mejia-domenzain_evolutionary_2022}), study the composition of plots, and whether to use absolute or relative values\footnote{The complete protocol is available in the supplementary materials.}.

% trim=left bottom right top  \fbox
\begin{figure}
    \centering 
    %\includegraphics[clip, trim=4.7cm 11.7cm 9.7cm 6.0cm, width=1\textwidth]{figures/method-3.pdf}
    \includegraphics[clip,width=1\textwidth]{figures/groups_comp-2.pdf}
    \caption{Examples of group comparison time series charts explored in the survey}
    \label{fig:comp}
\end{figure}

\noindent Lastly, to measure visualization literacy\cite{lee2016vlat}, we asked participants to solve four tasks adapted from VLAT \cite{lee2016vlat}: retrieve values (item 55), find extremum (item 2), find trend (item 38), and make comparisons with relative values (item 15). We analyzed the preferences differences based on demographics (sex and age) and personal factors (teaching level). We used the non-parametric test Kruskal–Wallis to evaluate the ordinal rankings. When significant, we performed a pairwise comparison using the Mann-Whitney U test, correcting for multiple comparisons via a Benjamini-Hochberg procedure.


\subsection{Results}

%Participants completed the study in 58 minutes (median time).
%% Graph literacy
\noindent \textbf{Graph Literacy}.  We computed the visualization literacy score (VL) as a weighted average using as weights the items' discrimination index times the content validity ratio from \cite{lee2016vlat} (0.6 for retrieving the value, 6 for finding extremum, 14 for finding trend, and 6.4 for making comparisons with relative values). The mean VL was 0.7/1.0 ($\sigma$ = 0.3) indicating good literacy. The personal (teaching level) and demographic (gender, age) factors did not explain the variance.  \\


% trim=left bottom right top  \fbox
\begin{figure}
    \centering 
    %\includegraphics[clip, trim=4.7cm 11.7cm 9.7cm 6.0cm, width=1\textwidth]{figures/method-3.pdf}
    \includegraphics[width=0.80\textwidth]{figures/results-2.png}
    \caption{Mean ranking for time series representation (a), and group comparison (b). (*) indicates a significant difference with \textit{p}-value $< 0.05$. }
    \label{fig:mean-ranking}
\end{figure}


%% Time series 
\noindent \textbf{Plot Type} \\
\noindent \textit{Time series}. We found that participants differed in their preferences to visualize time series behavior of students (${\chi}^2(5) = 188$, $p < 0.001$). For example, we used the \textit{Effort} feature of time spent online (e.g., see Figure \ref{fig:rank-effort}) and found that participants preferred (in ascending order where lower is better) bar plot ($\mu_{rank}$= 2.1), followed by bar plot with a line plot on top ($\mu_{rank}$=  2.7), a line plot with standard deviation (SD) ($\mu_{rank}$=  3.1), just a line plot ($\mu_{rank}$=  3.3), heat map ($\mu_{rank}$=  4.7) and box plot ($\mu_{rank}$= 4.9). As shown in figure \ref{fig:mean-ranking}a, university teachers ranked the line plot with SD higher ($\mu_{rank}$=  2.7) than the rest of the teachers (${\chi}^2(2) = 4.3$, $p = 0.03$). After the bar plot, it was the preferred plot. One of the main topics when explaining the preferences was \textit{clarity}. This is coherent with the findings from \cite{albers2014task} where the graph that included the bar plot with a line plot on top outperformed the other graphs (line plot, box plot, and heat map) at identifying statistical properties (e.g., range, average, extremes). However, when we analyzed the topics in the written insights derived from the plots, we found two topics (out of 13) unique to the heat map. Participants realized that \textit{usually most students were putting in 0 [effort]} and that \textit{a little amount of them spent a lot of time on the platform}. Although this information could have also been inferred from the line plot with standard deviation and the box plot, it is interesting that it was only mentioned for the heat map. \\

\noindent \textit{Frequency}. The preferences were similar when visualizing the frequency of events, for example, studying habits according to the day of the week and the time of the day. We found that 84\% of the participants preferred to visualize the frequency of events with a bar plot where the y-axis represented the frequency than with heat maps where the colors and the transparency illustrated the frequency. \\


%% Numerical proportion
\noindent \textit{Categorical}. To show the relative sizes of data, for example, the number of students per cluster at a given point, the pie chart ($\mu_{rank}$=  1.2) was strongly favored over a network graph ($\mu_{rank}$=  2.5), a stacked area graph ($\mu_{rank}$=  2.5), and a bubble chart ($\mu_{rank}$=  3.1). Participants argued that the pie chart \textit{is the most familiar and traditional}.\\

%% Comparison
\noindent \textbf{Group Comparison}}.
When comparing groups in graphs participants preferred superposition (overlaying objects in the same space) over juxtaposition (showing different objects separately). For example,  with time series line plots, 84\% of participants preferred superposition over juxtaposition (${\chi}^2(1) = 83$, $p < 0.001$). Likewise, when using bar plots to compare time series (see Figure \ref{fig:comp}), participants also preferred superposition over juxtaposition and the explicit encoding of relationships (${\chi}^2(3) = 67$, $p < 0.001$).  We explored superposition by overlapping objects side-by-side and on top of each other. As seen in Figure \ref{fig:mean-ranking}, side-by-side superposition was preferred ($\mu_{rank}$=  1.9) over juxtaposition ($\mu_{rank}$=  2.4), superposition on top of each other ($\mu_{rank}$=  2.6) and the difference between the time series ($\mu_{rank}$=  3.3). The participants of \textit{younger age} (younger than the 25th percentile of 30 years old) ranked the difference-between-time-series graph higher ($\mu_{rank}$=  2.9) than the rest of the participants ($\mu_{rank}$=  3.3) but it also remained as the lowest ranked. One \textit{young} participant noted that \textit{the difference makes it very simple as it reduces complexity (in terms of elements in the plot)}. However, despite explicit encodings can offload the burden of comparison from the viewer \cite{gleicher2011visual}, the preferred layout for time series was superposition. These findings were also valid for frequency plots where 83\% preferred superposition over juxtaposition.\\

%% Evolution of groups
\noindent \textbf{Group Evolution}. We compared graphs for the evolution of a numeric variable for several groups (see Figure \ref{fig:rank-profiles}) using a stacked area chart ($\mu_{rank}$=  1.5), a bubble chart ($\mu_{rank}$=  1.9) and a Sankey flow chart ($\mu_{rank}$=  2.6). Noteworthy, the participants of \textit{older age} (older than the 75th percentile of 46 years old) ranked the stacked area chart and the bubble chart equally ($\mu_{rank}$=  1.6), one of them noted \textit{the bubble charts were easier to read and understand the focus}. \\

\noindent \textbf{Plot Composition}. Moreover, we also studied the composition over time using stacked bar charts. We used, as example, the proportion of students per week that watched the pre-class videos before and after the interactive session. We found that 87\% of participants preferred having a third group with the students that did not watch the videos so that the bars would add up to the maximum number of students. Despite some participants argued that \textit{it isn't necessary to cluter the graph with that information}, the majority agreed that they \textit{would still prefer to see how many students did not watch than calculate it and add [their] head}. \\

%% Absolute or relative numbers
\noindent \textbf{Values Representation}. Participants were divided between showing the number of students as a percentage (51\%) or in absolute terms (49\%). However, 71\% of university teachers preferred percentages over absolute numbers, and some of them suggested \textit{adding the total number of students to the y-axis label so that it can be calculated with the percentages if desired}. Lastly, when comparing time series, we found that 75\% of the participants favored using legends in graphs. \\


\noindent \textit{In summary, teachers tend to prefer simpler and more familiar visualizations like bar plots and pie charts. In addition, when comparing groups the superposition layout was perceived as more useful. We found no differences regarding gender but found that age and teaching level (i.e., university) were correlated with some visual design preferences \textbf{(RQ1)}.}
 

==> sections/old/04-dashboard-study.tex <==
\section{Study 2: Teacher Dashboard for SRL Profiles}
\label{sec:dash-study}

To address \textbf{RQ2}, we design and implemented a teacher dashboard displaying SRL profiles and behaviors. We evaluate the tool with 10 teachers analyzing their clickstream, think-aloud process and semi-structured interview answers.

% trim=left bottom right top  \fbox
\begin{figure}
    \centering
    %\includegraphics[clip, trim=0.1cm 5.1cm 0cm 5.1cm, width=1\textwidth]{figures/overview.pdf}
    \includegraphics[width=0.8\textwidth]{figures/dashboard-design-2.png}
    \caption{Overview of pages: (a)\textit{Summary}, (b)\textit{Student Profiles}, (c) \textit{Effort} and (d) \textit{Effort groups} .}
    \label{fig:overview}
\end{figure}


\subsection{Design} From the user interviews, we designed and implemented a prototype of \texttt{FlippED}. We, then, iterated the design with seven university teachers. The final design includes a navigation menu (see F1 in Figure \ref{fig:overview}) with two parts: the overview (with the \textit{Summary} and the \textit{Student Profiles}) and the student behaviors (including \textit{Proactivity, Effort, Consistency, Control} and \textit{Regularity}). The user can select the course (F2) and the date range (F3). In addition, there are help buttons (F4) throughout the dashboard to clarify the different elements and to provide further explanations. Figure \ref{fig:overview} shows the two overview pages. In the \textit{Summary} page (left on Figure \ref{fig:overview}), weekly statistics per dimension are displayed as well as the trend in comparison to the previous week. The description of the profiles and the associated grades are shown on the \textit{Profiles} page (Figure \ref{fig:overview}b). Moreover, Figure \ref{fig:overview}c and \ref{fig:overview}d  show examples of the student behavior pages in which users can choose (F5) between the aggregated view (\ref{fig:overview}c) and a view per groups (\ref{fig:overview}d).


% trim=left botm right top  \fbox
%\begin{figure}
%    \centering
%    \includegraphics[clip, trim=1.9cm 12cm 5.5cm 6.3cm, width=1\textwidth]{figures/interaction.pdf}
%    \caption{Interaction flow.}
%    \label{fig:interaction-flow}
%\end{figure}


%The online interaction flow (see Figure \ref{fig:interaction-flow}) consists of retrieving the graphs, text, and captions from the database. Offline, the content retrieval backend obtains the students' clickstream data from the LMS and runs the clustering pipeline. The results are used to generate the graphs, text, and captions which are then stored in the database to be retrieved in real-time. \\

\noindent \textbf{Accessibility.} In order to make \texttt{FlippED} accessible to people with disabilities, we followed the guidelines from the \textit{Web Accessibility Initiative (WAI)} \cite{wai} and achieved the conformance level of AAA\footnote{The evaluation report is available in the supplementary materials.} (highest level). Some examples of accessible features include: using a colorblind palette and providing detailed alt-texts, and captions for all graphs; supporting dark contrast mode; and having a clear voice-navigable interface. 
The interface (frontend) was implemented with React and the content retrieval (backend) with FastAPI using a Postgres database. Both applications were hosted on Heroku.

\subsection{Experimental Setup}
\noindent \textbf{Participants}. We recruited 10 university-level teachers with experience in BL (6 had experience teaching FC), through a faculty email and LinkedIn posts. 50\% of the teachers identified as female. \\

%% Explain the survey (procedure)
\noindent \textbf{Procedure}. At the beginning of the user study, participants filled out a questionnaire about their trust in AI-based educational technology (EdTech). We used constructs 1, 3, and 5 (self-efficacy, anxieties, and benefits regarding AI-based EdTech) from \cite{nazaretsky_instrument_2022}. We then conducted semi-structured interviews where participants were given the same scenario from the visualization study: teaching a large FC university course. The first task was to follow a think-aloud protocol and explore the dashboard. After the exploration, participants were told that students had just taken their midterm exam and the results were surprisingly bad for some students. The second task was to use the dashboard to give possible explanations. Lastly, we asked participants to assess whether they would use it and how they would use it.


\subsection{Results}

% trim=left bottom right top 
\begin{figure}
    \centering
    \includegraphics[clip, trim=1cm 0cm 1cm 1cm, width=0.7\textwidth]{figures/flow.pdf}
    \caption{Clickstream of FlippED.}
    \label{fig:clickstream}
\end{figure}


\noindent \textbf{Interaction}. We analyzed the participants' exploration (task 1) clickstream and to study how much time was spent on each page and how the teachers navigated the dashboard. We complement the analysis with the participants' think-aloud comments. In Figure \ref{fig:clickstream}, each circle is a page and its area represents the time spent on each page on a logarithmic scale. The radius of the dark circle is the average time and the radius of the light circle is the average time plus the standard deviation. Participants spent the greatest time on the \textit{Profiles} page (10 minutes); half of the participants were at first confused about the profiles but then said they would go back to the \textit{Profiles} page regularly and use them to advise students on the best learning strategies. Moreover, they spent the least amount of time on the \textit{Consistency groups} page (2.3 minutes); they found the \textit{Consistency} page redundant with \textit{Effort}. 

Moreover, the transition probabilities are represented by the width and the transparency of the arrows on a linear scale. We only plotted the edges with a transition probability greater than 0.12 to visualize the most frequent transitions. The highest transition probability in Figure \ref{fig:clickstream} is from \textit{Control groups} to \textit{Regularity} ($p=1$) and the lowest is from \textit{Effort} to \textit{Effort groups} ($p=0.14$). In the beginning, as shown in Figure \ref{fig:clickstream, } participants started in the \textit{Summary} page and went into the \textit{Profiles} page or \textit{Proactivity}. Then participants, went back and forth to understand the layout and the profiles. Once it was clear, they followed mostly an ordered exploration strategy, they accessed the pages following the sequential order from the menu.  

In the second task, when asked to use the dashboard to identify possible causes for poor midterm performance, 80\% of the participants went to the \textit{Profiles} page and the remaining 20\% to the \textit{Summary} page and then to the \textit{Profiles} page. Then, participants described the qualities of the poor-performing profiles. Overall, participants knew where to find the information. However, they mentioned that \textit{there was a lot of information} and would most likely just check the \textit{Summary} and the \textit{Profiles} page on a regular basis rather than all the pages. \\
 

\noindent \textbf{Trust in AI}. Similar to \cite{nazaretsky_instrument_2022}, we used a 1-5 point scale (1 = "strongly agree", 5 = "strongly disagree" and 3 neutral) to measure three questions per construct. At the beginning of the interview, participants showed a high self-efficacy ($\mu = 3.8$) regarding using and trusting AI-based EdTech in their classroom, a low anxiety ($\mu = 2.3$) related to privacy and teaching autonomy in EdTech, and a slight awareness of the potential benefits ($\mu = 3.3$) of these tools including assisting teachers with in-class management activities, preparing lessons and assigning personalized tasks. 

Despite the low anxiety regarding EdTech, 60\% of the participants during the interview asked whether the data was anonymized and noted that students should be able to opt out if desired. Another concern mentioned was the loss of interaction with the students because the monitoring would be done automatically rather than by interacting with the students. \\

\textbf{Actionability}. Furthermore, regarding the potential benefits, 80\% of the participants said they would show the visualizations to the students. In particular, they mentioned adding the Proactivity graphs to the course slides, showing the link between profile and grade to encourage proactive behaviors. As one participant illustrated, \textit{I would also use this information as feedback to students on their working habits. [...] I would [show them this information] and say: 'Look, the success correlates. Why don't you try to change this?'}. Moreover, 70\% mentioned adapting the course in some way; some examples were: asking for questions before the interactive face-to-face sessions to force students to watch videos before the session, adapting the workload, adding activities such as quizzes, proposing additional materials, or switching to classical teaching if students don't seem to adapt well to the FC format. Other possible actions teachers mentioned were sending messages to all students with some recommendations, sending automatic reminders to students who are not working regularly, and advising students in the lowest-grade profile to change their learning strategies. 

\textit{In summary, teachers initially explored the dashboard in an iterative manner switching between the overview pages (\textit{Summary} and \textit{Profiles}) and the first page: \textit{Proactivity} because they struggled to understand the profiles and clusters. Then, they explored in a sequential manner. Teachers proposed actions like sharing the data with the students and adapting the course according to the graphs   \textbf{RQ2}.}

==> sections/old/srlprofiles.tex <==
\section{Multi-Dimensional SRL Profiles}
Recent work on BL and student behavior has focused on students' studying habits and SRL patterns \cite{saint2020, mejia-domenzain_identifying_2022}. \cite{mejia-domenzain_identifying_2022} studied SRL through 5 different lenses: \textit{Effort}, \textit{Consistency}, \textit{Regularity}, \textit{Control}, and \textit{Proactivity}. Different patterns of behaviors were identified using a multi-step time series clustering pipeline that takes as input clickstream features from a learning management system (LMS). The five lenses were integrated into multi-dimensional student profiles that are correlated with academic performance. Technically, \cite{mejia-domenzain_identifying_2022} measured \textit{Effort} with the time online and clicks on videos; \textit{Consistency} with the mean session duration and relative time online; \textit{Regularity} with the day-of-the-week and hour-of-the-day periodicity; \textit{Proactivity} with the delay or anticipation to watch the lecture content; and \textit{Control} using the pause frequency and the changes in video speed. In the pipeline, they (1) calculate the dynamic time-warping distance between the students' time series features, (2) add the distances from the features in the same dimension, and (3) use Spectral Clustering to find the different groups per dimension. In a second clustering step, the resulting labels per dimension (5 labels) are clustered using K-Modes. In our work, we adapt the clustering pipeline from \cite{mejia-domenzain_identifying_2022} to study how to communicate and visualize students' behaviors and ML-based profiles. \\

==> sections/together/02-method-together.tex <==
\section{Methodology}
To study how to best communicate online student behavior with teachers, we followed the participatory co-design approach shown in Figure \ref{fig:method}. We first conducted ten contextual interviews with university teachers to understand their needs and requirements in the context of FC. From the interviews, we grouped the requirements into visualization requirements (how they would like to visualize behaviors in graphs) and communication requirements (how they would like to receive and organize the information). Next, we designed graphs according to the users' requirements and literature guidelines \cite{gleicher2011visual,albers2014task}. 
To study the preferences of educators, we conducted a visualization study with 100 teachers (See Section \ref{sec:vis-study}). Afterward, we implemented the findings from the visualization study and adapted the graphs accordingly. In parallel, following the communication requirements, we designed a dashboard and then integrated the graphs resulting from the visualization study. We iteratively tested and modified the dashboard prototype with seven different university teachers. Finally, we evaluated the latest version of the dashboard with ten university teachers in a usability study (See Section \ref{sec:dash-study}). \\

% trim=left bottom right top  \fbox
\begin{figure}
    \centering 
    %\includegraphics[clip, trim=4.7cm 11.7cm 9.7cm 6.0cm, width=1\textwidth]{figures/method-3.pdf}
    \includegraphics[width=0.8\textwidth]{figures/method-6.png}
    \caption{Participatory co-design approach}
    \label{fig:method}
\end{figure}



\subsection{Contextual Understanding} 
\label{sec:context}

%% Introduce clustering pipeline (?)
\noindent \textbf{SRL Profiles}. 
Recent work on BL and student behavior has focused on students' studying habits and SRL patterns \cite{saint2020, mejia-domenzain_identifying_2022}. Previous work \cite{mejia-domenzain_identifying_2022} has studied SRL through 5 different lenses: \textit{effort}, \textit{consistency}, \textit{regularity}, \textit{control}, and \textit{proactivity}. Different patterns of behaviors were identified using a multi-step time series clustering pipeline that takes as input clickstream features from a learning management system (LMS). The five lenses were integrated into multi-dimensional student profiles that are correlated with academic performance. Technically, \cite{mejia-domenzain_identifying_2022} measured \textit{effort} with the time online and clicks on videos; \textit{consistency} with the mean session duration and relative time online; \textit{regularity} with the day-of-the-week and hour-of-the-day periodicity; \textit{proactivity} with the delay or anticipation to watch the lecture content; and \textit{control} using the pause frequency and the changes in video speed. In the pipeline, they (1) calculate the dynamic time-warping distance between the students' time series features, (2) add the distances from the features in the same dimension, and (3) use Spectral Clustering to find the different groups per dimension. In a second clustering step, the resulting labels per dimension (5 labels) are clustered using K-Modes. In our work, we adapt the clustering pipeline from \cite{mejia-domenzain_identifying_2022} to study how to communicate and visualize students' behaviors and ML-based profiles. \\


\noindent \textbf{Potential User Interviews}. We conducted semi-structured interviews with ten teachers at university level (50\% of the teachers identified as female). The median time of the interviews was 40 minutes. Participants were asked about their experience with blended learning and the challenges they encountered. Then, they were asked about the information they would have liked to know and how would they have liked to see or receive that information. Lastly, they were asked to make a sketch and draw how they would like the information to be visualized and organized.\\





\subsection{Visual Design Teacher Preferences} 
\label{sec:vis-method}

%% Participants
\noindent \textbf{Participants}.We recruited $100$ participants using Prolific, prescreening participants fluent in English and that taught in the education industry. We removed 8 participants that failed the attention checks. In addition, we requested a balanced sample of male and female participants (51\% female). The age of the respondents ranged between 21 and 76 years old, with a median of 37 years old. 68\% of the participants came from Europe and more precisely 41\% from the United Kingdom. 34\% of the participants reported teaching at university, 29\% at high school, 23\% at elementary school, and the remaining 14\% included kindergarten, adult education, and vocational education. We found that only 35\% of the university teachers were female. \\


%% Explain the survey (procedure)
\noindent \textbf{Procedure}. Participants were given the scenario of teaching a large university course for bachelor students in a flipped manner. They were told they had taught 2/3 of the course and would be shown visualizations of their students' behavior. Next, the participants were shown, in random order, graphs corresponding to each of the SRL dimensions \cite{mejia-domenzain_identifying_2022}. Per visualization, participants were asked to (1) describe and analyze the graph as if they had to explain it to a visually impaired colleague (the descriptions were used to generate the captions and alt-text), (2) explain their insights, and (3) suggest how to improve the graph (optional). In addition, to measure visualization literacy, we asked participants to solve four tasks adapted from VLAT \cite{lee2016vlat}: retrieve values (item 55), find extremum (item 2), find trend (item 38), and make comparisons with relative values (item 15).

\begin{figure}
    \centering
%\includegraphics[width=1.00\textwidth]{figures/plots_examples.png}
    \includegraphics[clip, trim=0.3cm 0.35cm 0.25cm 0.25cm, width=1\textwidth]{figures/plots_examples.pdf}
    \caption{Examples of time series visual designs explored in the survey.}
    \label{fig:rank-effort}
\end{figure}

Furthermore, we asked participants to rank in ascending order (rank 1 is the highest and best) different types of graphs for a single feature according to their usefulness and explain the rationale for their preference. Similar to \cite{albers2014task}, we visualized time series using different designs and graph types. For example, Figure \ref{fig:rank-effort} shows a bar plot, line plot, box plot, and heat map to represent the time the students spent on online activities through time. We explored other visual designs for the evolution of groups (e.g., stacked area graph, bubble graph, and Sankey flow graph in Figure \ref{fig:rank-profiles}) and design decisions including whether it is more useful to show the relative or the absolute number of students, and use of legends\footnote{The complete protocol is available in the supplementary materials.}. Lastly, like \cite{gleicher2011visual}, we explored comparative designs of multiple time series including juxtaposition, superposition, and explicit encoding of relationships.
% trim=left bottom right top  \fbox
\begin{figure}
    \centering
    \includegraphics[clip, trim=0.9cm 18.3cm 2.8cm 2.0cm, width=1\textwidth]{figures/profiles-examples.pdf}
    \caption{Examples of charts for the evolution of groups explored in the survey.}
    \label{fig:rank-profiles}
\end{figure}


%Visual Design Teacher Preferences
\subsection{Teacher Dashboard for SRL Profiles} 
\label{sec:dash-method}

% trim=left bottom right top  \fbox
\begin{figure}
    \centering
    %\includegraphics[clip, trim=0.1cm 5.1cm 0cm 5.1cm, width=1\textwidth]{figures/overview.pdf}
    \includegraphics[width=1\textwidth]{figures/dashboard-design.png}
    \caption{Overview of pages: (a)\textit{Summary}, (b)\textit{Student Profiles}, (c) \textit{Effort} and (d) \textit{Effort groups} .}
    \label{fig:overview}
\end{figure}


\noindent \textbf{Design}. From the potential user interviews, we designed and implemented a prototype of \texttt{FlippED}. The design includes a navigation menu (see F1 in Figure \ref{fig:overview}) with two parts: the overview (with the \textit{Summary} and the \textit{Student Profiles}) and the student behaviors (including \textit{Proactivity, Effort, Consistency, Control} and \textit{Regularity}). The user can select the course (F2) and the date range (F3). In addition, there are help buttons (F4) throughout the dashboard to clarify the different elements and to provide further explanations. Figure \ref{fig:overview} shows the two overview pages. In the \textit{Summary} page (left on Figure \ref{fig:overview}), weekly statistics per dimension are displayed as well as the trend in comparison to the previous week. The description of the profiles and the associated grades are shown on the \textit{Profiles} page (Figure \ref{fig:overview}b). Moreover, Figure \ref{fig:overview}c and \ref{fig:overview}d  show examples of the student behavior pages in which users can choose (F5) between the aggregated view (\ref{fig:overview}c) and a view per groups (\ref{fig:overview}d).

The online interaction flow (see Figure \ref{fig:interaction-flow}) consists of retrieving the graphs, text, and captions from the database. Offline, the content retrieval backend obtains the students' clickstream data from the LMS and runs the clustering pipeline. The results are used to generate the graphs, text, and captions which are then stored in the database to be retrieved in real-time. \\

% trim=left botm right top  \fbox
\begin{figure}
    \centering
    \includegraphics[clip, trim=1.9cm 12cm 5.5cm 6.3cm, width=1\textwidth]{figures/interaction.pdf}
    \caption{Interaction flow.}
    \label{fig:interaction-flow}
\end{figure}

\noindent \textbf{Accessibility.} In order to make \texttt{FlippED} accessible to people with disabilities, we followed the guidelines from the \textit{Web Accessibility Initiative (WAI)} \cite{wai} and achieved the conformance level of AAA\footnote{The evaluation report is available in the supplementary materials.} (highest level). Some examples of accessible features include: using a colorblind palette and providing detailed alt-texts, and captions for all graphs; supporting dark contrast mode; and having a clear voice-navigable interface. 
The interface (front-end) was implemented with React and the content retrieval (back-end) with FastAPI using a Postgres database. Both applications were hosted on Heroku.


\noindent \textbf{Participants}. We recruited 10 university-level teachers with experience in BL (6 had experience teaching FC), through a faculty email and LinkedIn posts. 50\% of the teachers were female. \\

%% Explain the survey (procedure)
\noindent \textbf{Procedure}. At the beginning of the user study, participants filled out a questionnaire about their trust in AI-based educational technology (EdTech). We used constructs 1, 3, and 5 (self-efficacy, anxieties, and benefits regarding AI-based EdTech) from \cite{nazaretsky_instrument_2022}. We then conducted semi-structured interviews where participants were given the same scenario from the visualization study: teaching a large FC university course. The first task was to follow a think-aloud protocol and explore the dashboard. After the exploration, participants were told that students had just taken their midterm exam and the results were surprisingly bad for some students. The second task was to use the dashboard to give possible explanations. Lastly, we asked participants to assess whether they would use it and how they would use it.


\subsection{Measures and Analysis}


\noindent \textbf{ML-Assisted Analysis}
We recorded with consent all the semi-structured interviews (contextual interviews and user studies) and transcribed them using \texttt{Whisper} \cite{radford2022robust}, a state-of-the-art zero-shot model for speech recognition. We then performed the qualitative analysis assisted by topic modeling. We identified the main topics using \texttt{BERTopic}~\cite{grootendorst2022bertopic}, a topic modeling technique that integrates the contextual information of the text by clustering embeddings generated by pre-trained Transformer-based language models. In particular, we generated the embeddings using \texttt{Sentence-BERT}~\cite{reimers2019sentence}. The code and supplementary materials (e.g., interview protocols) are available at \url{https://anonymous.4open.science/r/flipped/}. \\

\noindent \textbf{Ranking Analysis.} For the Visual Design Teacher Preferences, we analyzed the preferences differences based on demographic (sex and age) and personal factors (teaching level). We used the non-parametric test \textit{Kruskal–Wallis} to evaluate the ordinal rankings. When significant, we performed a pairwise comparison using the \textit{Mann-Whitney U} test, correcting for multiple comparisons via a \textit{Benjamini-Hochberg (BH)} procedure.



==> sections/together/03-results.tex <==

\section{Results}

\noindent \textbf{Potential User Interviews}. Most teachers interviewed agreed that having data about their students' learning behaviors would help them adapt their course and give personalized feedback to specific student profiles. The most mentioned requirement was anonymous data and aggregated statistics. Educators were concerned about data privacy and shared ethical concerns. However, they showed interest in general group statistics. For example, 60\% of the interviewees mentioned it would be useful to know whether students viewed the material, how much time they spent watching the videos, and the number of students keeping up with the class. Some other mentions were students’ consistency in watching the videos, whether students worked at the last minute before an exam, and the average video playback speed. \\ 

\subsection{Visual Design Teacher Preferences}
%% Graph literacy
Participants completed the study in 58 minutes (median time). We computed the visualization literacy score (VL) as a weighted average using as weights the items' discrimination index times the content validity ratio from \cite{lee2016vlat} (0.6 for retrieving the value, 6 for finding extremum, 14 for finding trend, and 6.4 for making comparisons with relative values). The mean VL was 0.7/1.0 ($\sigma$ = 0.3) indicating good literacy. The personal and demographic factors did not explain the variance.  

We found that participants differed in their preferences to visualize time series behavior of students (${\chi}^2(5) = 188$, $p < 0.001$). We used the \textit{Effort} feature of time spent online (e.g., see Figure \ref{fig:effort}) and found that participants preferred (in ascending order where lower is better) bar-plot ($\mu_{rank}$= 2.1), followed by bar plot with a line plot on top ($\mu_{rank}$=  2.7), a line plot with standard deviation ($\mu_{rank}$=  3.1), just a line plot ($\mu_{rank}$=  3.3), heat map ($\mu_{rank}$=  4.7) and box plot ($\mu_{rank}$= 4.9). Interestingly, university teachers ranked the line plot with standard deviation higher ($\mu_{rank}$=  2.7) than the rest of the teachers (${\chi}^2(2) = 4.3$, $p = 0.03$). After the bar plot, it was the preferred plot.

One of the main topics when explaining the preferences was \textit{clarity}. This is coherent with the findings from \cite{albers2014task} where the graph that included the bar plot with a line plot on top outperformed the other graphs (line plot, box plot, and heat map) at identifying statistical properties (e.g., range, average, extremes). However, when we analyzed the topics in the written insights derived from the plots, we found two topics (out of 13) unique to the heat map. Participants realized that \textit{usually most students were putting in 0 [effort]} and that \textit{a little amount of them spent a lot of time on the platform}. Although this information could have also been inferred from the line plot with standard deviation and the box plot, it is interesting that it was only mentioned for the heat map.


Participants were divided between showing the number of students as a percentage (51\%) or in absolute terms (49\%). However, 71\% of university teachers preferred percentages over absolute numbers, and some of them suggested \textit{adding the total number of students to the y-axis label so that it can be calculated with the percentages if desired}. In addition, we compared graphs for the evolution of a numeric variable for several groups (see Figure \ref{fig:rank-profiles}) using a stacked area chart ($\mu_{rank}$=  1.5), a bubble chart ($\mu_{rank}$=  1.9) and a Sankey flow chart ($\mu_{rank}$=  2.6). Noteworthy, the participants of \textit{older age} (older than the 75th percentile of 46 years old) ranked the stacked area chart and the bubble chart equally ($\mu_{rank}$=  1.6), one of them noted \textit{the bubble charts were easier to read and understand the focus}.

Moreover, when comparing time series, we found that 75\% of the participants favored the use of legends in graphs. In addition, with line plots, 84\% of participants preferred superposition (overlaying objects in the same space) over juxtaposition (showing different objects separately) (${\chi}^2(1) = 83$, $p < 0.001$). Furthermore, when using bar plots to compare time series, participants also preferred superposition over juxtaposition and the explicit encoding of relationships (${\chi}^2(3) = 67$, $p < 0.001$).  We explored superposition by overlapping objects side-by-side and on top of each other. We found that side-by-side superposition was preferred ($\mu_{rank}$=  1.9) over juxtaposition ($\mu_{rank}$=  2.4), superposition on top of each other ($\mu_{rank}$=  2.6) and the difference between the time series ($\mu_{rank}$=  3.3). The participants of \textit{younger age} (younger than the 25th percentile of 30 years old) ranked the difference-between-time-series graph higher ($\mu_{rank}$=  2.9) than the rest of the participants ($\mu_{rank}$=  3.3) but it also remained as the lowest ranked. One \textit{young} participant noted that \textit{the difference makes it very simple as it reduces complexity (in terms of elements in the plot)}; this observation is in line with \cite{gleicher2011visual} that argues that explicit encodings can offload the burden of comparison from the viewer. 

\subsection{Teacher Dashboard for SRL Profiles}

% trim=left bottom right top 
\begin{figure}
    \centering
    \includegraphics[clip, trim=1cm 0cm 1cm 1cm, width=1\textwidth]{figures/flow.pdf}
    \caption{Clickstream of FlippED.}
    \label{fig:clickstream}
\end{figure}



\noindent \textbf{Exploration tasks}. We analyzed the participants' exploration (task 1) clickstream to study how much time was spent on each page and how the teachers navigated the dashboard. In Figure \ref{fig:clickstream}, each circle is a page and its area represents the time spent on each page on a logarithmic scale. The radius of the dark circle is the average time and the radius of the light circle is the average time plus the standard deviation. Participants spent the greatest time on the \textit{Profiles} page (10 minutes); half of the participants were at first confused about the profiles but then said they would go back to the \textit{Profiles} page regularly and use them to advise students on the best learning strategies. Moreover, they spent the least amount of time on the \textit{Consistency groups} page (2.3 minutes); they found the \textit{Consistency} page redundant with \textit{Effort}. 


Moreover, the transition probabilities are represented by the width and the transparency of the arrows on a linear scale. We only plotted the edges with a transition probability greater than 0.12 to visualize the most frequent transitions. The highest transition probability in Figure \ref{fig:clickstream} is from \textit{Control groups} to \textit{Regularity} ($p=1$) and the lowest is from \textit{Effort} to \textit{Effort groups} ($p=0.14$).\\

In the second task, when asked to use the dashboard to identify possible causes for poor midterm performance, 80\% of the participants went to the \textit{Profiles} page and the remaining 20\% to the \textit{Summary} page and then to the \textit{Profiles} page. Then, participants described the qualities of the poor-performing profiles. \\
 

\noindent \textbf{Trust in AI}. Similar to \cite{nazaretsky_instrument_2022}, we used a 1-5 point scale (1 = "strongly agree", 5 = "strongly disagree" and 3 neutral) to measure three questions per construct. At the beginning of the interview, participants showed a high self-efficacy ($\mu = 3.8$) regarding using and trusting AI-based EdTech in their classroom, a low anxiety ($\mu = 2.3$) related to privacy and teaching autonomy in EdTech, and a slight awareness of the potential benefits ($\mu = 3.3$) of these tools including assisting teachers with in-class management activities, preparing lessons and assigning personalized tasks. 

Despite the low anxiety regarding EdTech, 60\% of the participants during the interview asked whether the data was anonymized and noted that students should be able to opt out if desired. Another concern mentioned was the loss of interaction with the students because the monitoring would be done automatically rather than by interacting with the students. 

Furthermore, regarding the potential benefits, 80\% of the participants said they would show the visualizations to the students. In particular, they mentioned adding the Proactivity graphs to the course slides, showing the link between profile and grade to encourage proactive behaviors. As one participant illustrated, \textit{I would also use this information as feedback to students on their working habits. [...] I would [show them this information] and say: 'Look, the success correlates. Why don't you try to change this?'}. Moreover, 70\% mentioned adapting the course in some way; some examples were: asking for questions before the interactive face-to-face sessions to force students to watch videos before the session, adapting the workload, adding activities such as quizzes, proposing additional materials, or switching to classical teaching if students don't seem to adapt well to the FC format. Other possible actions teachers mentioned were sending messages to all students with some recommendations, sending automatic reminders to students who are not working regularly, and advising students in the lowest-grade profile to change their learning strategies. 

==> tables/procedure-vis-3.tex <==
\begin{tabular}{@{}p{2.5cm}p{3cm}p{6.7cm}@{\hskip 0.5cm}p{3cm}@{}}
\toprule
\textbf{Concept} &
  \textbf{Feature Type} &
  \textbf{Description} &
  \textbf{Tasks} \\ \midrule
\textit{Plot Type} &
  Time series &
  Different designs (bar plot, bar plot with a line plot on top, line plot with SD, line plot, heat map and box plot). &
  Interpret (heat map, line plot with SD); rank and explain \\
 &
  Frequency &
  Different designs (bar plot and heat map). &
  Interpret (bar plot, heat map); rank and explain. \\
 &
  Categorical &
  Different designs (pie chart, network graph, stacked area chart and bubble chart). &
  Rank and explain \\
  \midrule
\textit{Group Comparison} &
  Time series &
  Different layouts (superposition, juxtaposition and explicit encoding of relationships) for line plot and bar charts. &
  Rank and explain \\
 &
  Frequency &
  Different layouts (superposition and juxtaposition) for bar charts. &
  Rank and explain \\
\midrule
\textit{Group Evolution} &
  Categorical time series &
  Different designs (stacked area chart, bubble chart, Sankey chart). &
  Rank and explain \\
    \midrule
\textit{Plot Composition} &
  Categorical time series &
  Different composition (selected groups, all groups). &
  Rank and explain \\
    \midrule
\textit{Value Representation} &
  Categorical &
  Different representations (absolute number or percentage). &
  Rank and explain \\ \bottomrule
\end{tabular}%

==> tables/procedure-vis.tex <==


\begin{tabular}{@{}p{3cm}p{3cm}p{6.7cm}@{\hskip 0.5cm}p{3cm}@{}}
\toprule
\textbf{Concept \mbox{Explored}} & \textbf{Type of data}   & \textbf{Evaluation}                                                                & \textbf{Preference} \\ \midrule
\textit{Representation} &
  Time series &
  Different designs (bar plot,  bar plot with a line plot on top,  line plot with standard deviation, just a line plot, heat map and box plot). &
  Bar plot \\
\textit{}                 & Frequency               & Different designs (bar plot and heat map).                                         & Bar plot            \\
\textit{}                 & Categorical             & Different designs (pie chart, network graph, stacked area chart and bubble chart). & Pie chart           \\
\textit{}                 & Categorical \mbox{time series} & Different designs (stacked area chart, bubble chart, Sankey chart) and different composition (selected groups, all groups)                & Stacked area chart  \\
\textit{}                 & Values                  & Different representations (absolute number of percentage)                          & No clear preference \\
\midrule
\textit{Group Comparison} &
  Time series &
  Different layouts (superposition, juxtaposition and explicit encoding of relationships) for line plot and bar charts. &
  Superposition (side-by-side) \\
                          & Frequency               & Different layouts (superposition and juxtaposition) for bar charts.                & Superposition       \\ \bottomrule
\end{tabular}%


==> tables/procedure_vis_long.tex <==
\begin{tabular}{@{}p{1.8cm}p{1.8cm}p{7cm}p{1.7cm}@{}}
\toprule
\textbf{Concept} & \textbf{Data Type} & \textbf{Description (Items)} & \textbf{Dimension} \\ 
\midrule
\textit{Plot Type} & Time series & Describe ($e_1$: heat map, $e_2$: line plot with SD) & Effort \\ 
%&& $e_2$: Describe (line plot with SD) & \\
&& Rank ($e_3$: bar plot, bar plot with line, line plot, line plot with SD, heat map, box plot) & \\
&& Describe ($c_1$: line plot with SD) & Consistency \\
\noalign{\vskip 1mm}    
& Frequency &  Describe ($r_1$: heat map, $r_2$: bar plot) & Regularity \\
& & Choose ($r_3$: bar plot or heat map) & \\ 
\noalign{\vskip 1mm}
& Categorical & Rank ($p_1$: pie/stacked area/bubble chart, network graph) & Profiles \\
\midrule
\textit{Comparison} & Time series & Rank (superposition, juxtaposition, or explicit encoding for $e_6$: line plot and $e_7$: bar plot) & Effort \\
\noalign{\vskip 1mm}
& Frequency & Describe ($r_4$: bar plot, comparing two groups) & Regularity \\
& & Rank ($r_5$: bar plot superposition, juxtaposition, explicit encoding) & \\
\midrule
\textit{Composition} & Time series & Rank ($p_2$: stacked area/bubble/Sankey chart) & Profiles \\
& & Describe ($a_1$: show selected groups or all groups) & Proactivity \\
&& Choose ($a_2$: show selected groups or all groups) & \\
&& Choose ($a_3$: show positive/negative values) & \\
\midrule
\textit{Plot Details} & Time series & Choose (bar plot: $e_4$:legend/no legend, $e_5$: one vs. multiple features) & Effort \\
\noalign{\vskip 1mm}
& Frequency & Choose ($a_4$: absolute/relative values) & Proactivity \\
\noalign{\vskip 1mm}
 & Categorical & Choose ($p_3$: absolute/relative values) & Profiles \\ 
\bottomrule
\end{tabular}%

==> tables/procedure_vis_new.tex <==


\begin{tabular}{@{}p{3cm}p{3cm}p{6.7cm}@{\hskip 0.5cm}p{3cm}@{}}
\toprule
\textbf{Concept \mbox{Explored}} & \textbf{Type of data}   & \textbf{Evaluation}                                                                & \textbf{Preference} \\ \midrule
\textit{Representation} &
  Time series &
  Different designs (bar plot,  bar plot with a line plot on top,  line plot with standard deviation, just a line plot, heat map and box plot). &
  Bar plot \\
\textit{}                 & Frequency               & Different designs (bar plot and heat map).                                         & Bar plot            \\
\textit{}                 & Categorical             & Different designs (pie chart, network graph, stacked area chart and bubble chart). & Pie chart           \\
\textit{}                 & Categorical \mbox{time series} & Different designs (stacked area chart, bubble chart, Sankey chart) and different composition (selected groups, all groups)                & Stacked area chart  \\
\textit{}                 & Values                  & Different representations (absolute number of percentage)                          & No clear preference \\
\midrule
\textit{Group Comparison} &
  Time series &
  Different layouts (superposition, juxtaposition and explicit encoding of relationships) for line plot and bar charts. &
  Superposition (side-by-side) \\
                          & Frequency               & Different layouts (superposition and juxtaposition) for bar charts.                & Superposition       \\ \bottomrule
\end{tabular}%

==> tables/procedure_viz_4.tex <==
\begin{tabular}{@{}p{1.8cm}p{1.8cm}p{1.9cm}p{1.5cm}p{6cm}@{}}
\toprule
\textbf{Dimension} & \textbf{Type} & \textbf{Concept} & \textbf{Task} & \textbf{Items} \\
\midrule
\textbf{P}rofiles & Categorical & \textit{Plot Type} & Rank  & $p_1$: pie/stacked area/bubble/network chart \\
& &  \textit{Composition} & Rank  & $p_2$: stacked area/bubble/Sankey chart \\
& &  \textit{Plot Details} & Choose & $p_3$: absolute/relative values\\ 
\midrule
\textbf{E}ffort & Time series & \textit{Plot Type} & Interpret & $e_1$: heat map, $e_2$: line plot with SD \\
& & & Rank & $e_3$ (Fig. \ref{fig:rank-effort}): bar plot w/ and w/o line, line plot w/ and w/o SD, heat map, box plot\\
 & & \textit{Plot Details} & Choose & $e_4$, $e_5$: legend use, number of features  \\
& & \textit{Comparison} & Rank & $e_6$, $e_7$ (Fig. \ref{fig:comp}): layouts for bar/line plots \\
\midrule
\textbf{C}onsistency & Time series & \textit{Plot Type} & Interpret &$c_1$: line plot with SD\\
\midrule
\textbf{R}egularity & Frequency & \textit{Plot Type} &  Interpret & $r_1$: heat map, $r_2$: bar plot  \\
& & & Choose & $r_3$: bar plot, heat map\\ 
&  & \textit{Comparison} & Interpret & $r_4$: bar plot with two groups\\
& & & Rank & $r_5$ (cf. Fig. \ref{fig:comp}): layouts for bar plots\\
\midrule
Pro\textbf{a}ctivity & Time series & \textit{Composition} & Interpret & $a_1$: stacked bar chart \\
&&& Choose & $a_2$: show few groups or all groups (100\%) \\
&& \textit{Plot Details} & Choose & $a_3$: absolute/relative values \\
\bottomrule
\end{tabular}%
